Distributional MIPLIB: a Multi-Domain Library for Advancing ML-Guided MILP Methods

Mixed Integer Linear Programming (MILP) is a fundamental tool for modeling combinatorial optimization problems. Recently, a growing body of research has used machine learning to accelerate MILP solving. Despite the increasing popularity of this approach, there is a lack of a common repository that provides distributions of similar MILP instances across different domains, at different hardness levels, with standardized test sets. In this paper, we introduce Distributional MIPLIB, a multi-domain library of problem distributions for advancing ML-guided MILP methods. We curate MILP distributions from existing work in this area as well as real-world problems that have not been used, and classify them into different hardness levels. It will facilitate research in this area by enabling comprehensive evaluation on diverse and realistic domains. We empirically illustrate the benefits of using Distributional MIPLIB as a research vehicle in two ways. We evaluate the performance of ML-guided variable branching on previously unused distributions to identify potential areas for improvement. Moreover, we propose to learn branching policies from a mix of distributions, demonstrating that mixed distributions achieve better performance compared to homogeneous distributions when there is limited data and generalize well to larger instances. The dataset is publicly available at https://sites.google.com/usc.edu/distributional-miplib/home.

==> neurips_data_2023/related_work_extended_version.tex <==
\subsection{Introduction}


In today's rapidly evolving society and economy, the scale, pace, and variety of tasks related to resource allocation, design, planning, and operations are expanding. These tasks are often subject to stringent resource constraints, heightened quality expectations, and increasingly complex environments. For instance, the design and operations of large-scale supply chains, disrupted by phenomena such as hurricanes, wildfires, winter storms, and pandemics like COVID-19, critically impact the well-being of communities and the stability of markets and economies. Central to addressing these challenges is the resolution of complex optimization problems that typically require both discrete and continuous decision-making. TODO: SHORTEN THIS PARAGRAPH TO ONE SENTENCE?



%Today's society and economy face an ever-increasing scale, pace, and variety of tasks related to resource allocation, design, planning and operations, while often subjected to tighter resource constraints, higher expectations for quality, and more complex environments.  For example, the design and operations of large-scale supply chains in a world affected by increasing disruptions, such as hurricanes, wildfires, winter storms or even pandemics like COVID-19, may affect the well-being of entire communities and the stability of the markets and economy. At the heart of all of these challenges is the constant need of solving optimization problems that often involve a combination of discrete and continuous decisions. 


Mixed Integer Linear Programming (MILP) represents one of the most essential techniques for modeling and solving combinatorial optimization problems across various domains, including e-commerce \cite{greening2023lead} and energy systems \cite{kody2022optimizing}. MILPs are inherently challenging to solve; their combinatorial nature often renders gradient-based methods ineffective. Both the artificial intelligence (AI) and operations research (OR) communities have developed robust optimization systems to tackle these problems. However, as the problems scale in size, complexity, and real-time demands, traditional optimization technologies encounter significant challenges. To facilitate advancements in solvers and methodologies,  \cite{miplib2017} release MIPLIB, which is a diverse collection of more than a thousand of challenging real-world MILP instances from various
academic and industrial applications suited for benchmarking and testing of MILP solvers.
%solving large-scale MILPs remains a formidable task. advancements in 


Recent research  blends algorithmic strategies with machine learning techniques to tailor new, problem-specific policies. This approach is motivated by the observation that similar MILP models, which often share structural similarities, are repeatedly solved across various applications \cite{amos2023tutorial}. In particular, a growing body of literature enhances traditional algorithmic frameworks, such as the branch-and-bound method and large neighborhood search for MILP, with adaptable learning components that leverage data and training. Instead of relying on a standard benchmark such as MIPLIB, most existing research formulates MILP instances independently. One of the main reason is that MIPLIB instances are too diverse in difficulties, structures and sizes, and machine learning approaches are still yet incapable of learning policies that generalize well to diverse MILP instances. In Table \ref{tabl}



%Mixed Integer Linear Programming is one of the most fundamental techniques for modelling and solving combinatorial optimization problems, covering various application domains such as e-commerce \citet{greening2023lead} and energy systems \citet{kody2022optimizing}. 
%MILPs are hard to solve, and gradient-based methods are typically not applicable because of their combinatorial nature. The AI and OR communities have long and rich track records of developing optimization systems to solve
%these problems. However, as problems grow in size, complexity, and real-time requirements, existing optimization technology faces tremendous challenges. Despite development in solvers and techniques, solving large-scale MILP remains challenging. Instead of designing solution methods purely as a challenge in algorithm design and mathematical insight, a new paradigm of research combines algorithmic ideas and insights with machine learning approaches to discover new policies customized to the problem types and instance distributions that appear in specific applications, motivated by the fact that similar MILP models that share similar structures are solved repeatedly in many applications \cite{ding2020accelerating} (this provides opportunity for mL). In particular, a growing body of research augments well-established and effective algorithmic frameworks (such as branch-and-bound search in mathematical programming) with learning components that are inherently customizable with data and training.

This paper introduces {\it Distributional MIPLIB}, a comprehensive, multi-purpose MILP library encompassing a variety of MILP problem distributions aimed at supporting the development of machine learning-guided MILP-solving methods. The rationale for creating this dataset includes: (1) the current practice where researchers independently formulate instances and distributions, leading to a lack of standardized datasets for comparative analysis; Synthetic and small-scale instances are often used in publications.  (2) the intention to advance research by enabling evaluations across broader domains and facilitating novel research tasks that explore multi-domain, multi-task learning; and (3) the significant contributions of ML-guided MILP solving to the OR field, highlighting the synergistic potential of integrating AI and OR. This platform will not only foster collaboration among researchers in discrete optimization and machine learning but also provides a repository for submitting MILP instances that could benefit from ML-driven solutions. It aims to offer a unique resource for ML researchers to access MILP problems of varying sizes and complexities, including real-world scenarios, thereby promoting research that requires minimal domain-specific knowledge. 


%We provide a large-scale, multi-purpose dataset comprising multiple domains of MILP distributions, aiming to facilitate research on the development of machine learning-guided MILP-solving methods. The motivations of this library are: (1) Currently, everyone formulates instances and distributions on their own. There is a lack of a standard set for people to compare between different approaches
%(2) We hope to open a new avenue for research by strengthening within one task by evaluating on more domains and facilitating new tasks (towards learning shared representation: multi-domain, multi-task)
%(3) The growing body of research on ML-guided MILP solving has contributed significantly to OR and exemplifies how fusing AI and OR may lead to synergistic effects that could not have been realized otherwise. We hope to provide a platform that connects the OR and AI community, by helping ML researchers get access to MILP problems with different sizes and difficulty as well as real-world instances
%A platform for researchers to submit instances that can potentially benefit from ML. The research needed to achieve this requires close collaborations between researchers in discrete optimization, global optimization, combinatorial optimization, machine learning, and computational science/algorithm design. 

%- allow researchers to use instances without domain knowledge for some real-world instances...
%- great for different tasks because of the variety of size and domain: MILP instances cater to various ML tasks on learning to optimize MILPs. 

Overview of dataset: We compiled a set of xxx distributions (List of domains, real-world vs classical). Benchmarks: how are they organized: train/test/val; generators; metrics: nodes, runtime, primal-dual integrals

 

1. limited set of domains
2. hard to benchmark
3. three-four domains have been repeatedly used



\begin{itemize}
    \item distributional
    \item Diverse
    \item Real-world  Synthetic
\end{itemize}

\paragraph{the potential for training mixed model}

\paragraph{Comparison with Existing Datasets and Contributions.}
Current work suffers from one or more of the following drawbacks: (1) does not contain a large number of instances for the same distribution (MIPLIP); (2) does not contain a wide range of distributions (TSPLIB) (3) focuses on ML-for-MILP with specific tracks such as learning to configure solvers (MIPLEARN), reinforcement learning (or-gym), and learning inside solvers (Ecole). (4) not having real-world instances

Moreover, we include real-world instances...

ML methods typically benefit from a large number of training data points from the same distribution (same type of problem), but existing libraries (such as MIPLIB) contain a relatively small number of instances for each problem type


\subsection{Different Tasks of ML for MILP}

There are many components for decision-making within BnB, including 
preprocessing, cutting planes, branching rules, and primal heuristics,
which are typically hand-crafted and hard-coded aimed at improving the performance over a large class of benchmarks. Once devised,
these hard-coded strategies are essentially input-agnostic. Departing from this established approach, data-driven techniques have
shown great promise in bringing significant performance
improvements. 
\paragraph{Learning to Branch} 

%for which the LP solution is a fractional (denoted as $\bar{x_i}$) and thus violates the integrality constraints. The algorithm creates one subproblem by adding the constraint $x_i \leq \floor{\bar{x_i}}$ to $Q'$ to the left branch and the other by adding the constraint $x_i \geq \ceiling{\bar{x_i}}$ to the right branch. 
%The algorithm prunes a branch if the corresponding subproblem is infeasible or it obtains a proof that the optimal solution of the subproblem cannot be better than the best one discovered so far. 

 A series of papers %have explored data-driven approaches to learning branching heuristics that improve solving times.
%\cite{balcan2018learning,gasse2019exact,khalil2016learning,nair2020solving}.
 %It is now possible to 
 have explored learning to branch by imitating the strong branching heuristic, a branching method that results in fewer search tree nodes but is expensive to compute ~\cite{khalil2016learning,lodi2017learning,alvarez2017machine,balcan2018learning,gasse2019exact,gupta2020hybrid,nair2020solving,lin2024cambranch}. The strong branching heuristic computes a score for each branching candidate and these methods either learn to predict the variables' score or learn to rank them according to their scores. %using data collected either offline over similar instances and on the fly while solving a particular instance %\cite{khalil2016learning,alvarez2017machine,lodi2017learning,gupta2020hybrid}. Much of the literature on improving variable selection using ML is based on imitating strong branching, a branching policy that results in fewer search nodes but is time-consuming ~\cite{khalil2016learning,lodi2017learning,alvarez2017machine,balcan2018learning,gasse2019exact,gupta2020hybrid,nair2020solving,lin2024cambranch}. 
For the features and ML models, \cite{khalil2016learning} develop the first ML-based framework for learning to branch using a Support Vector Machine (SVM) with hand-crafted features. \cite{gasse2019exact} extend the framework by using a bipartite graph to encode the MILP and  Graph Convolution Networks (GCN) to learn variable representations. %[TODO: write more about the bipartite graph repreesntation]

%The unifying trend in prior work is to approximate ``strong branching'', an expensive but informative look-ahead procedure, with a ML proxy in the spirit of ``learning to optimize''. While strong branching has a solid foundation and empirical evidence support in mathematical programming, it may be far from optimal \cite{dey2021theoretical}, and is still myopic as it uses a one-step look-ahead. There is thus an opportunity to use machine learning to discover branching policies from experience, which would deviate from current practices, take into account delayed effects, and lead to new performance improvements.



% This algorithm implicitly enumerates all solutions while using the linear programming relaxation of the subMILPs to rule out suboptimal regions in the search space. The algorithm terminates when it has pruned every leaf and returns the best solution obtained. As the size of the tree can be affected by variables that are branched on at each iteration, variable selection in the branching step is a parameter that practitioners tune to improve the performance of the algorithm.






\paragraph{Learning Backdoors}

Backdoor for MILPs is a small subsets of variables such that a
MILP can be solved optimally by branching \textit{only} on
the variables in the set \cite{williams2003backdoors}. Therefore, identifying backdoors efficiently and effectively can greatly improve the performance of B\&B. \cite{ferber2022backdoors} using ML to predict the most effective backdoor candidates generated by a LP relaxation-based sampling methods. More recently, \cite{cai2024learning} propose to use a Monte-Carlo tree search method \cite{khalil2022finding} to improve the quality of training data and apply contrastive learning to directly construct backdoors   %from are most critical for specific distributions of instances. [TODO: add more references]

%This observation supports the strong focus of improving branching and, in particular, using machine learning to recognize which variables are most critical for a specific instance. 
%Backdoors do not arise in ``synthetic'' benchmarks and is present in some practical applications \cite{Dilkina2007,Dilkina2009,Dilkina2009a}.  

%Backdoors for MILPs are defined as small subsets of variables such that prioritizing branching on them whenever possible leads to faster running times. However, finding high-quality backdoors that improve running times remains an open question. Previous work learns to estimate the relative solver speed of randomly sampled backdoors through ranking and then decide whether to use it \cite{ferber2022learning}. 
% In our work, we utilize the Monte-Carlo tree search method \cite{khalil2022finding} to collect backdoors for training, rather than relying on random sampling, and adapt a contrastive learning framework to train a Graph Attention Network model to predict backdoors.


\paragraph{Learning Primal Heuristics}
Primal heuristics refer to routines that find good feasible solutions in a short amount of time \cite{BolusaniEtal2024OO} and 
%are instrumental in finding high-quality solutions early. However, not all primal heuristics have a high chance of success and, therefore, 
deciding which heuristics to run and when is an important task. These decisions are mostly made by hard-coded frequency rules in MILP solvers, which are static, instance-oblivious, and context-independent. To tackle this challenge, \cite{khalil2017primalheuristics} propose a  data-driven approach to decide when to execute primal heuristics. \cite{chmiela2021learning} derive a data-driven approach for scheduling primal heuristics.

Another line of research is to learn to predict solutions to MILPs. Both \cite{nair2020solving} and \cite{han2023gnn}
learn to predict optimal solutions to  MILPs and fix the values for a subset of variables based on the prediction to get  reduced-size MILPs that are faster to solve. 

%[TODO: another line of research is to solution prediction]
\paragraph{Large Neighbourhood Search (LNS)} LNS is a meta-heuristic that can find high quality solutions faster than B\&B on large-scale MILP instances but provides no optimality guarantees. It starts with a feasible solution to the MILP and iteratively selects a subset of variables to reoptimize. %Designing the right heuristics to maximize the performance of LNS remains an open problem. 
  Local Branching (LB) is a heuristic that finds the variables that lead to the largest improvement over the current solution in each iteration of LNS. But LB is often slow since it needs to solve a MILP of the same size as input. To mitigate this issues, \cite{sonnerat2021learning} and \cite{huang2023searching}  replace LB with imitation-learned policies. Other ML techniques, such as reinforcement learning (RL), have also been applied to learn destroy heuristics for LNS \cite{song2020general,wu2021learning}.
%We follow this line of research and first proposes a classic heuristic based on Local Branching (LB) \cite{huang2023local}. LB is a heuristic that selects the neighborhood that leads to the largest improvement over the current solution in each iteration of LNS. LB is often slow since it needs to solve an ILP of the same size as input. Our proposed heuristics, LB-RELAX and its variants, use the linear programming relaxation of LB to select neighborhoods. We evaluate LB-RELAX on four benchmarks, namely, the minimum vertex cover, maximum independent set, multiple knapsack and set covering problems. These instances have up to 9,000 variables and 45,000 constriants. With an hour runtime limit, it improves the solution quality (measured by the primal gap) by 41\% - 100\% and the speed of improving solutions (measured by the primal integral) by 33\% - 84\% when compared against the best baselines.

%We also propose CL-LNS to learn such heuristics with contrastive learning \cite{huang2023searching}. In this work, we learn via imitating LB following \citet{sonnerat2021learning} and improve the performance by contrasting positive and negative examples of selected variable subsets. We evaluate CL-LNS on four benchmarks, namely, the minimum vertex cover, maximum independent set, combinatorial auction and set covering problems. These instances have up to 12,000 variables and 135,100 constraints. With an hour runtime limit, it improves the solution quality (measured by the primal gap) by 31\% - 95\% and the speed of improving solutions (measured by the primal integral) by 32\% - 59\% when compared against the previous state-of-the-art ML-guided approaches.
\paragraph{Learning to Cut}
A cutting-plane is a constraint that is valid for feasible integer solutions but cuts into the feasible region of the linear programming (LP) relaxation, thus improving the bound on the optimal solution. Adding cutting planes has been shown to speed up B\&B \cite{bixby:ro:2007,dey2021lower}. Modern MILP solvers maintain a cut-pool that includes a large number of cutting planes of a diverse set of classes. The decisions regarding which classes of cutting planes to use, as well as the specific cutting planes to select from each class, significantly impact solver performance. In recent advancements, \cite{tang2020reinforcement} introduce a RL framework tailored for the Gomory cutting-plane algorithm. Additionally, \cite{huang2022learning} develop a method to approach cut selection as a learning-to-rank task, while \cite{paulus2022learning}  devise a strategy to imitate a lookahead strategy for cut selection.
%, e.g., Chv\'atal-Gomory cuts~\cite{Gomory58}, Gomory mixed-integer cuts ~\cite{gomory:1960b}, mixed-integer rounding inequalities ~\cite{nemhauser:wo:1990}, clique cuts~\cite{johnson:pa:1982}. 
%Decisions on which cutting-plane classes to use and which set of cutting planes to add from each class can impact the solvers' performance. %, and the solving time depends on the specific MILP instance. 
%Cut-pool management rules in MILP solvers are mostly input agnostic and not take into account the structure of MILP instances. Improving cutting-plane selection in a data-driven fashion using ML can lead to dramatic improvements in solvers.
%\cite{tang2020reinforcement} propose a RL framework for the Gomory cutting plane algorithm. \cite{huang2022learning} learn cut selection as a learning-to-rank task. \cite{paulus2022learning} learn to imitate a lookahead strategy for cut selection. %applying this method to a proprietary solver


%Cutting planes are added in the root node before branching or at any other part of the B\&B search tree. Selecting cuts is not an easy task: too many cuts slow down the LP solver and too few cuts causes the B\&B tree to be much larger. 



\subsection{Existing Libraries and Software Packages}

There are a few instance libraries built for different combinatorial optimization problems. 
MIPLIB \cite{miplib2017} is a library of  MIP instances that provides access to real-world mixed integer programs. It contains 1065 instances that are diverse in sizes, structures, difficulties, and underlying problem domains, and has become a standard test set used to compare the performance of MILP solvers. Several ML methods for MILP solving have been tested on MIPLIB instances \cite{sonnerat2021learning,wu2021learning,li2024learning}. Despite some early success, it remains great challenges for ML methods to deliver state-of-the-art performance across problem domains. In contrast, Distributional MIPLIB provides a test bed for developing ML methods for in-distribution tasks as well as out-of-distribution generalization. %A subset of 240 instances was specially selected for benchmarking solver performance3.
TSPLIB \cite{reinelt1991tsplib} is a library of instances for the Travelling Salesman Problem (TSP) and related problems. It provides a diverse set of instances, allowing researchers to develop and benchmark their algorithms against a wide range of TSP variants. 

There are also a few software packages built to facilitate research in ML-guided combinatorial optimization. Closely relate to our work is Ecole \cite{prouvost2020ecole}, designed to facilitate the integration of machine learning in combinatorial optimization solvers. It exposes the sequential decision-making process that must be perform in MILP solving as Markov Decision Processes and allows ML models to work in cooperation with an open-source MILP solver that acts as a controllable algorithm. MIPLEARN \cite{santos_xavier_2024_10627485} is another software package for ML-guided MILP solving that provides access to a complete ML pipeline including data collection, training, and testing. Both Ecole and MIPLEARN provide MILP generators for synthetic problems which can be used for compiling distributional MILP instances.  OR-Gym  \cite{HubbsOR-Gym} is an open-source software for developing RL algorithms for combinatorial optimization which  models and solves classic optimization problems as RL tasks. %OR-Gym provides a new ML tool for the OR community, while also opens the RL community to many of the problems and challenges in OR.

\iffalse
\begin{itemize}
    \item or-gym: A Reinforcement Learning Library for Operations Research Problems
    \item MIPLEARN: for learning to configure solvers %https://anl-ceeesa.github.io/MIPLearn/0.4/
    \item TSPLIB: a library of sample instances for the TSP (and related problems) 
    \item Ecole
    \item MIPLIB \cite{gleixner2021miplib} provides a heterogeneous set of instances coming from diverse applications. To foster progress on ML-based MIP solvers, the project will compile a
library of instances motivated by the iconic MIPLIB library. MIPLIB
has consistently driven progress in MIP solvers by providing a common
repository for challenging models. No counterpart for the MIPLIB
exists for distributional settings which aim at collecting similar
instances of the same model. 
\end{itemize}
from diverse applications.

\fi

